PLUE: Language Understanding Evaluation Benchmark for Privacy Policies in English

Privacy policies provide individuals with information about their rights and how their personal information is handled. Natural language understanding (NLU) technologies can support individuals and practitioners to understand better privacy practices described in lengthy and complex documents. However, existing efforts that use NLU technologies are limited by processing the language in a way exclusive to a single task focusing on certain privacy practices. To this end, we introduce the Privacy Policy Language Understanding Evaluation (PLUE) benchmark, a multi-task benchmark for evaluating the privacy policy language understanding across various tasks. We also collect a large corpus of privacy policies to enable privacy policy domain-specific language model pre-training. We evaluate several generic pre-trained language models and continue pre-training them on the collected corpus. We demonstrate that domain-specific continual pre-training offers performance improvements across all tasks.

==> tables/hyperparams.tex <==
\begin{table*}[!th]
    % \small
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c c }
    \toprule
    & \textbf{PP-BERT} & \textbf{PP-SpanBERT} & \textbf{PP-Electra} & \textbf{PP-RoBERTa}\\ \midrule
    Learning Rate & 1e-4 & 1e-4 & 1e-4  & 6e-4\\
    Train Steps & 100,000 & 100,000 & 100,000 & 12,500 \\
    batch Size & 256 & 256 & 256 & 2048 \\
    Learning Rate Schedule & linear & polynomial\_decay & linear & linear \\
    \# warm-up steps & 1000 & 1000 & 1000 & 600 \\
    Optimizer & AdamW & AdamW & AdamW & AdamW \\
    \bottomrule
    \end{tabular}
    % }
    \caption{Hyperparameters for pre-training language models.}
    \label{tab:pretraining_hyperparams}
\end{table*}
% \bigskip
\begin{table*}[!th]
    % \small
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular} {l  c  c  c  c  } % {l | c | c | c | c | c | c | c | c }
    \toprule
    & \makecell{\textbf{Text}\\\textbf{Classification}}  & \makecell{\textbf{Question}\\\textbf{Answering}} & \makecell{\textbf{Semantic}\\\textbf{Parsing}} &\makecell{\textbf{NER}} \\
    \midrule
    Dropout & 0.1 & 0.1 & 0.1 & 0.1 \\
    Weight decay & 0.0 & 0.0 & 0.0 & 0.0 \\
    Optimizer & AdamW & AdamW & AdamW & AdamW \\
    Batch Size & 32 & 32 & 32 & 32 \\
    Learning rate & \multicolumn{4}{c}{[3e-4, 1e-4, 5e-5, 3e-5, 1e-5, 5e-6, 3e-6]} \\
    Learning Rate Schedule & Linear & Linear & Linear & Linear \\
    Warm-up Ratio & 0.05 & 0.0 & 0.05 & 0.05 \\
    \# epoch & 20 & 3 & 20 & 20 \\
    \bottomrule
    \end{tabular}
    % }
    \caption{Hyperparameters for fine-tuning pre-trained language models on different PLUE tasks.}
    \label{tab:finetuning_hyperparams}
\end{table*}

